Priorities in gravitational waveforms for future space-borne detectors: vacuum accuracy or environment?

In preparation for future space-borne gravitational-wave (GW) detectors, should the modelling effort focus on high-precision vacuum templates or on the astrophysical environment of the sources? We perform a systematic comparison of the phase contributions caused by 1) known environmental effects in both gaseous and stellar matter backgrounds, or 2) high-order post-Newtonian {(PN)} terms in the evolution of mHz GW sources {during the inspiral stage of massive binaries}. We use the accuracy of currently available analytical waveform models as a benchmark {value, finding} the following trends: the largest unmodelled phase contributions are likely environmental rather than PN for binaries lighter than $\sim 10^7/(1+z)^2$~M$_{\odot}$, where $z$ is the redshift. Binaries heavier than $\sim 10^8/(1+z)$~M$_{\odot}$ do not require more accurate {inspiral} waveforms due to low signal-to-noise ratios (SNRs). For high-SNR sources, environmental {phase contributions} are relevant at low redshift, while high-order vacuum templates are required at $z > 4$. Led by these findings, we argue that including environmental effects in waveform models should be prioritised in order to maximize the science yield of future mHz detectors.

==> answer.tex <==
Dear anonymous reviewer,

We thank you for the very detailed report, that has led us to improve our draft significantly. Before addressing the bullet points individually, we would like to start with a general overview of the changes in the text (in red) and a clarification on the intended methodology.

The original draft of this work was intended to be a short letter (5 pages of text + 1 page of references), which forced us to be very succinct. The reviewer rightly points out many paragraphs in which this brevity came at the cost of clarity, perhaps creating some misunderstandings. In this revision, we attempted to explain our approach and our methodology in more detail throughout the paper, adding approximately 1 full page of text and taking care to address the reviewer's points where required.

The goal of our paper is not to determine the bias in parameter estimation caused by environmental effects using a specific waveform model. Rather, we wish to provide a general framework to estimate their importance for, crucially, any type of waveform, both analytical and numerical. To achieve this, we used a simple but plausible phenomenological model for the phase evolution (eq. 2) and compared the effects of vacuum PN orders against several types of environmental effects.

We hope that the referee sees the utility in this type of approach after the many revisions we added to the text.

Additionally, the page limit forced us to be very sparing with references. The reviewer rightly points out many cases in which our bibliography was incomplete, and we have added approximately 30 references accordingly throughout the whole text.

We think that this effort has led to a significantly improved version of our work, without requiring to change its intended spirit: a phenomenological analysis of environmental effects, short and easily comprehensible to both the astrophysics and relativity communities interested in GWs and LISA. Therefore, we warmly thank the anonymous reviewer for the thoroughness of the report.

Sincerely,
Lorenz Zwick et al.

Point by point response:

Points 1) and 2):
--Line 45: not clear what next-to-leading order dynamics means. Next order in what quantity?
--Line 52: "leading order parameters". Again, it is unclear what leading order (in what quantity?) means

We attempted to rephrase and clarify the whole introduction, removing mentions to "leading order" parameters.

Point 3):
--Page 1, second column: "pushing analytical approximations to higher and higher orders." Not clear what analytic approximations (PN? self force? EOB? Phenom?) the authors have in mind. I think a discussion of waveform models and the techniques (including numerical ones) used to obtain them would be of order here.

We attempted to rephrase and clarify this point in the red paragraph in the second column of page 1.

Point 4):
--Page 1, second column: further references on the bias/loss of parameter estimation accuracy due to environmental effects e.g.  1702.06529, 1907.02018, 2010.06056, 2205.08550, 2207.10086, 2001.03620, 0711.4558

We added several references including most the above throughout the text.

Point 5)
--Page 1 "these deviations represents a unique opportunity to measure properties of the source’s environment": another motivation is to test GR (for which environmental effects are foregrounds). This point was made, quantitatively, in 1404.7149 (already cited)

Added mention to GR in the sentence above.

Point 6)
--In eq 2, the remainder should be O(v/c)2 and not O(v/c) (there is no 0.5 PN order in GR!)

We addressed the issue. Moreover, we mistakenly reported the formula in the limit of small mass ratios in the paper while using the complete one in our code.

Point 7) to 11):
--Below eq 2, left column (discussion of the state of the art of waveform modeling). As mentioned above, the authors do not discuss at all numerical relativity, EOB/Phenom waveforms etc, and focus on PN waveforms. Those are NOT appropriate for massive BH binaries, which seem the focus here judging from fig 1.
--I do not know what is meant by "The step up to 5-PN accuracy has also been achieved by calibrating against numerical relativity simulations." If the authors think about the EOB, the goal of the latter is NOT to obtain the 5PN dynamics, but rather the waveforms in the inspiral, merger and ringdown (the last two extending beyond the PN approximation). I do not think anyone claims that you can extract the real 5PN dynamics from the EOB or from NR simulations...
--Eq 3 is only valid in the PN approximation. As I mentioned above, for massive black hole binaries PN waveforms are NOT sufficient. They are instead sufficient for stellar origin black holes in LISA, see arXiv:1811.01805. I suggest the authors focus on those sources in the next revision.
--On page 2, why do the authors work with the characteristic strain? It is much more common to write the SNR in terms of the Fourier transform of the waveform. More importantly, eq 5 and 6 are approximations only valid 1) at the leading 0PN order and 2) for quasi-monochromatic binaries (eq 6). This is definitely not sufficient for massive black hole binaries and *not even for stellar origing black holes*
--The criterion given by eq 8 is very simplistic, see arXiv:1811.01805 for a better one. The crucial point is that eq 8 does not involve any marginalization on the initial phase and merger time (which is required to assess the impact of environmental effects for parameter estimation, see arXiv:1811.01805) or over the whole set of source parameters (this latter marginalization is needed if one wants to assess the impact of environmental effects for detection). In fact, it is not clear at all if the authors are looking at the impact of environmental effects on detection or parameter estimation

We have attempted to collectively address these points by significantly clarifying the methodology and the limitations of our approach.

Point 12) 13) and 14):
--"Less typical environmental influences such as dark matter or other baryonic fields have also been explored in the literature": much additional work in this direction has been done by Brito, Cardoso, Pani and collaborators.
--"The presence of a third body can induce tidal fields and/or linear accelerations": references are needed here. some (on the acceleration) are mention in point #4 above, while for the effect of a third body on the waveforms see arXiv:1707.04902, arXiv:1812.01011
--Regarding the Doppler shift on page 3, see arXiv:2205.08550

We attempted to address these points by adding several references along with significant clarifications throughout section 2.2.

Point 15):
--On page 4 the authors attempt to identify an "effective PN order": I think this concept is misleading at it is at best valid in the inspiral only, while the waveforms for massive black holes are not PN waveforms. I suggest the authors restrict their analysis to stellar origin black hole binaries and stick to mismatch calculations like in arXiv:1811.01805

Considering that our analysis is limited to the inspiral phase, we would argue that such a concept is quite useful as a simple comparison tool between the accuracy of arbitrary vacuum waveforms and the expected phase shifts caused by environmental effects. We attempted to clarify its utility in the text. We also changed the name to "comparative" PN order for clarity. 


Point 16):
--On page 4: "sources with the highest SNRs land around a total mass of ∼ 106 M⊙ and mass ratio of <∼ 0.2. In this range, environmental influences are detectable at low redshift (z <∼ 2), while high-order vacuum corrections dominate at z ∼ 5.". I do not think the authors can conclude anything about detectability since they are not marginalizing over at least initial phase and merger time (see again arXiv:1811.01805)

We attempted to reword and clarify our conclusions in light of our methodology.

Point 17):
--Sec 3.2: there is much more work on environmental effects on EMRIs, see point #4

We added over 30 references throughout the text, including on this point.

